ToddlerDiffusion: Interactive Structured Image Generation with Cascaded Schr\"odinger Bridge

Diffusion models break down the challenging task of generating data from high-dimensional distributions into a series of easier denoising steps. Inspired by this paradigm, we propose a novel approach that extends the diffusion framework into modality space, decomposing the complex task of RGB image generation into simpler, interpretable stages. Our method, termed ToddlerDiffusion, cascades modality-specific models, each responsible for generating an intermediate representation, such as contours, palettes, and detailed textures, ultimately culminating in a high-quality RGB image. Instead of relying on the naive LDM concatenation conditioning mechanism to connect the different stages together, we employ Schr\"odinger Bridge to determine the optimal transport between different modalities. Although employing a cascaded pipeline introduces more stages, which could lead to a more complex architecture, each stage is meticulously formulated for efficiency and accuracy, surpassing Stable-Diffusion (LDM) performance. Modality composition not only enhances overall performance but enables emerging proprieties such as consistent editing, interaction capabilities, high-level interpretability, and faster convergence and sampling rate. Extensive experiments on diverse datasets, including LSUN-Churches, ImageNet, CelebHQ, and LAION-Art, demonstrate the efficacy of our approach, consistently outperforming state-of-the-art methods. For instance, ToddlerDiffusion achieves notable efficiency, matching LDM performance on LSUN-Churches while operating 2$\times$ faster with a 3$\times$ smaller architecture. The project website is available at: https://toddlerdiffusion.github.io/website/

==> Figures/5_sketch_palete_data.tex <==
% --------------------------------------------------------
\begin{figure}[t!]
\captionsetup{font=scriptsize}
\begin{minipage}[c]{.45\linewidth}
    %\vspace{0pt}
    \begin{center}
        \includegraphics[width=0.9\linewidth]{Figures/1st_forward_process.pdf}
        \captionof{figure}{Comparison between different formulations for the $1^{st}$ stage. This depicts the forward process for each formulation.}
        \label{fig_1st_forward_process}
    \end{center}
\end{minipage}
\begin{minipage}[c]{.54\linewidth}
    %\vspace{0pt}
    \begin{center}
        \includegraphics[width=0.98\linewidth]{Figures/Palette_pipeline.pdf}
        \captionof{figure}{Palette generation pipeline. First, we employ FastSAM \cite{zhao2023fast} to segment the image. Then,  we get the dominant color for each segment.}
        \label{fig_palette_pipeline}
    \end{center}
\end{minipage}
\vspace{-5mm}
\end{figure}
% --------------------------------------------------------

==> Figures/tex/del_exp_SamplingSteps.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%    Figure      %%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t!]
    \captionsetup{font=scriptsize}
    \centering
        \begin{minipage}{.3\linewidth}
            \includegraphics[width=\textwidth]{Figures/figures/1ststage_trainingsteps.png}
        \end{minipage}
        \begin{minipage}{.3\linewidth}
            \includegraphics[width=\textwidth]{Figures/figures/2ndstage_trainingsteps.png}
        \end{minipage}
        \begin{minipage}{.3\linewidth}
            \includegraphics[width=\textwidth]{Figures/figures/sampling_steps_trimming.png}
        \end{minipage}

        % Shared caption for first two images
        \begin{minipage}{0.65\textwidth}
            \centering
            \captionof{figure}{Ablation study for trimming the denoising steps during training and sampling. On the left is the results for the $1^{st}$ stage and on the right is the results for the $2^{nd}$ stage.}
        \end{minipage}\hfill
        % Caption for the third image
        \begin{minipage}{0.3\textwidth}
            \centering
            \captionof{figure}{Training steps ablation study on LSUN-Churches dataset.}
        \end{minipage}
    \label{fig_Denoising_Time_Steps_ablation}
    \vspace{-1em}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%    Figure      %%%%%%%%%%%%%%%%%%%%

==> Figures/tex/exp_ImgNetRobust_andControlSD.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%    Figure      %%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
    \captionsetup{font=scriptsize}
    \centering
        \begin{minipage}{.49\linewidth}
            \includegraphics[width=1\textwidth]{Figures/figures/NIPS_rebuttal_ImagenetResults.pdf}
            \captionof{figure}{Our results on the ImageNet dataset. The first column depicts the input sketch. The diagonal (green) represents the generated output that follows the sketch and the GT label. The off-diagonal images show the output given the sketch and inconsistent label. These adversarial labels show our model's robustness, where the successful cases are in yellow, and the failure ones are in red.}
            %\vspace{-1.0em}
            \label{fig_exp_ImageNetRobust}
        \end{minipage}
        \begin{minipage}{.49\linewidth}
            \includegraphics[width=0.99\textwidth]{Figures/figures/Controlability_SD.pdf}
            \vspace{-1.0em}
            \captionof{figure}{Comparison between our method and other baselines that enables sketch conditioning for SD-v1.5.}
            %\vspace{-1.0em}
            \label{fig_exp_conditioningSD1.5}
        \end{minipage}
        \vspace{-1.0em}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%    Figure      %%%%%%%%%%%%%%%%%%%%

==> sections/2_related.tex <==
\section{Related Work}
\label{sec_related_work}

Our novel architecture draws success from several areas, including diffusion models, chain-of-thought, and efficiency.

% --------------------------------------
\noindent \textbf{Efficient diffusion-based models.}
While diffusion models exhibit outstanding performance, they are burdened by significant training and inference costs, particularly when dealing with large-scale, high-resolution image datasets. The majority of research efforts have been spent on enhancing the sampling efficiency of these models. Some studies~\cite{lu2022dpm, karras2022elucidating, song2020denoising} have refined the sampling strategy using sophisticated numerical solvers, while others~\cite{salimans2022progressive, meng2023distillation, song2023consistency} have employed distillation to train a smaller network. Nonetheless, these methods don't directly address the challenge of reducing the training expenses associated with diffusion models. 
To achieve superior training efficiency, \cite{rombach2022high} suggests training a latent-space diffusion model by initially converting high-resolution images into a low-dimensional latent space.
% backbone
Regarding model architecture, recent developments like DiT~\cite{peebles2023scalable} and U-ViT~\cite{bao2023all}, grounded in the LDM framework, have transitioned from the U-Net~\cite{ronneberger2015u} backbone to the ViT~\cite{dosovitskiy2020image} backbone. This shift not only simplifies the model's architecture but also bolsters its training efficiency. 
% masked transformer
Models such as MDT~\cite{gao2023masked} and MaskDiT~\cite{zheng2023fast}, which are built upon the DiT framework, incorporate the masked transformer to expedite the training process, saving much training cost. 
% training method
The approach of \cite{wang2023patch} presents a novel patch-level training framework, capitalizing on the principles of patch-based training to maximize data use and heighten training efficiency.

\cite{song2020denoising, lu2022dpm, li2023snapfusion}

% --------------------------------------
\noindent \textbf{Chain of thoughts.}
The concept of a chain-of-thought has found applications across diverse machine learning domains, such as natural language processing \citep{wei2022chain, chowdhery2022palm, lyu2023faithful, wang2022self, zhang2023multimodal, madaan2022text}, robotics \citep{jia2023chain, yang2022chain}, and 3D visual grounding \cite{bakr2023cot3dref}. 
In the realm of text-image generation, recent benchmarks \cite{bakr2023hrs} have underscored various limitations. Addressing these concerns, recent works \cite{lian2023llm, balaji2022ediffi} have demonstrated the efficacy of decomposing the problem into sub-problems. 
%For a more comprehensive exploration of related works, an extended version is available in the supplementary materials.
%\cite{ho2022cascaded, huang2023composer}


==> sections/3_revisit.tex <==
\section{Revisiting Diffusion Models}
\label{sec_revisit}

% ----------------------------
\subsection{Preliminaries}

% 1)
Diffusion models~\cite{sohl2015deep,ho2020denoising,song2020score} progressively transform a sample $\mathbf{x}_0$ originating from a natural data distribution $\mathbf{x}_0 \sim q(\mathbf{x})$ into a noisy variant $\mathbf{x}_t$, i.e., forward process, where $t \in [1, T]$ and $T$ is the total number of the steps. The forward process~\cite{ho2020denoising} could be formulated by:
{\small
\begin{equation}
\label{eq_forward_process_ddpm}
    q\left(\mathbf{x}_t \mid \mathbf{x}_0\right)=\mathcal{N}\left(\mathbf{x}_t ; \sqrt{\bar{\alpha}_t} \mathbf{x}_0,\left(1-\bar{\alpha}_t\right) \mathbf{I}\right),
\end{equation}
}
where, $\sigma^{2}_t$ is the variance schedule, $\alpha_t=1-\sigma^{2}_t \text { and } \bar{\alpha}_t=\prod_{i=1}^t \alpha_i$.
Then, the goal is to learn the inverse mapping 
$q\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t\right)$
to be able to sample real data $\mathbf{x}_{0}$ given a Gaussian noise $\mathbf{x}_{T}$, i.e., reverse process.
However, this conditional probability is not tractable. 
Therefore, we approximate it using a model $p_\theta\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t\right)$, where $\theta$ represents the network parameters.
The learning objective is the Variational Lower Bound (ELBO):
\tao{bold x}

{\scriptsize
\begin{equation}
\mathcal{L}_{ELBO} = -\mathbb{E}_q\big(D_{KL}(q(x_T | x_0) || p(x_T)) + \sum^T_{t=2}D_{KL}(q(x_{t-1} | x_t, x_0) || p_{\theta}(x_{t-1} | x_t)) - \log p_{\theta}(x_0 | x_1)\big),
\label{ELBO_org}
\end{equation}
}

where the reverse process \cite{ho2020denoising} is formulated as:
{\scriptsize
\begin{equation}
\label{eq_reverse_process_ddpm}
q\left(x_{t-1} \mid x_t, x_0\right)=\mathcal{N}\left(\mathbf{x}_{t-1} ; \tilde{\mu}\left(\mathbf{x}_t, \mathbf{x}_0\right), \tilde{\sigma}^{2}_t \mathbf{I} \right)
\end{equation}
}

% ----------------------------
\subsection{Limitations}
% 1)
\noindent\textbf{Interpretability}
Diffusion-based methods lack interpretability in their denoising steps, making understanding the rationale behind the model's final image generation challenging. 
The hidden transformations in intermediate steps lack specific semantic meaning, hindering the attribution of contributions to overall image content \cite{deja2022analyzing}.

\noindent\textbf{Controllability}
The inherent lack of interpretability in diffusion-based methods limits controllability during image generation. 
Users struggle to exert direct control over specific attributes or features due to intricate denoising step transformations. 
To address this, we decompose the generation problem into multiple stages (Figure \ref{fig_teaser_forward_steps}), creating a Chain-of-Thoughts (CoT) framework.
CoT enables real-time monitoring and intervention in the generation process for complete control \cite{ju2023humansd}.

\noindent\textbf{Training time}
Current diffusion-based models suffer from prolonged training times, hampering their applicability, especially in resource-intensive tasks like video generation. This extended training period poses financial and environmental challenges. 
In contrast, our framework, {\papernameAbbrev}, achieves comparable performance to LDM while being 2x faster and using a 3x smaller architecture.

==> sections/6_discussion_lim.tex <==
\section{Discussion and Limitations}

\noindent \textbf{Social Impact}


\noindent \textbf{Text-to-Image}

Talk about how beneficial it is to solve the limitations in T2I models from the first stage only
